Time as it could Be measured in Artificial Living Systems

Being able to measure time, whether directly or indirectly, is a significant advantage for an organism. It permits it to predict regular events, and prepare for them on time. Thus, clocks are ubiquitous in biology. In the present paper, we consider the most minimal abstract pure clocks and investigate their characteristics with respect to their ability to measure time. Amongst other, we find fundamentally diametral clock characteristics, such as oscillatory behaviour for local time measurement or decay-based clocks measuring time periods in scales global to the problem. We include also cascades of independent clocks ("clock bags") and composite clocks with controlled dependency; the latter show various regimes of markedly different dynamics.

==> data/dragged_counter_tradeoff.tex <==
\begin{tikzpicture}
\begin{axis}[
    xlabel=Information Flow Constraint,
    ylabel=Mutual Information,
    xmin=0, xmax=1,
    ymin=1.4,ymax=2
    % ymin=1.5,ymax=2
]

\addplot [] table[x index=0, y index=1] 
    {data/drag_n9_mi_condmi_a.dat};
\addplot [] table[x index=0, y index=1] 
    {data/drag_n9_mi_condmi_b.dat};
\addplot [] table[x index=0, y index=1] 
    {data/drag_n9_mi_condmi_c.dat};
\end{axis}
\end{tikzpicture}





	

==> figs/parameter_cloud.tex <==
\begin{tikzpicture}
\begin{axis}[axis on top,
  xmin=0,xmax=1,ymin=0,ymax=2,
%   colorbar,
%   colormap/bluered,
  xlabel=Information Flow,
  ylabel=Mutual Information,
  x=6.54cm,y=4.38cm/2
%   x=5cm,y=4cm/2
]
\addplot graphics [xmin=0,xmax=1,ymin=0,ymax=2]
  {figs/parameter_cloud_n9_bw.png};
\end{axis}
\end{tikzpicture}
